Information-Theoretic Scaling Laws for Generative Diffusion Training

Diffusion models trained on increasingly large datasets sampled from the same data distribution will converge to the same learned distribution. However, in practice, a model trained on finite data depends on the particular training dataset; this dependence is reflected in properties of the model's outputs, such as memorization and sample quality. To understand this dependence through an information-theoretic lens, we study \textit{model information}, a computationally tractable measure of how much samples from the trained model depend on the particular training dataset. We explore its scaling behavior as model size and training dataset size vary. Specifically, we uncover two qualitatively distinct scaling regimes: (1) a nonlinear model information regime marking the transition from pure memorization to imperfect generalization, and (2) a generalization regime characterized by linear scaling of the model information and progressively improved generalization and sample quality. We then posit an information-theoretically principled scaling law to quantify these two regimes, and show that this law yields induced scaling laws for memorization and sample quality. We finally demonstrate that these induced scaling laws extrapolate well outside the fit's domain. Our results demonstrate information-theoretic principles for memorization and sample quality scaling laws in diffusion models. Our code is publicly available on \href{https://github.com/DruvPai/diffusion_info_theory_scaling_law}{GitHub}.

==> figures/pgfplots/edm_styles.tex <==
\providecolor{edmDepthOne}{RGB}{68,1,84}
\providecolor{edmDepthTwo}{RGB}{59,82,139}
\providecolor{edmDepthThree}{RGB}{33,145,140}
\providecolor{edmDepthFour}{RGB}{94,201,98}
\providecolor{edmDepthFive}{RGB}{230,205,28}
\providecolor{edmSetWarm}{RGB}{198,80,40}

\providecommand{\edmMetricSeries}[4]{%
  \addplot[
    color=#2,
    mark=#3,
    mark size=1.7pt,
    line width=0.75pt,
    mark options={solid, fill=#2, draw=#2},
    error bars/.cd,
    y dir=both,
    y explicit
  ] table[x=x,y=mean,y error=se,col sep=comma] {#1};
  \addlegendentry{#4}
}

\providecommand{\edmMetricSeriesNoLegend}[3]{%
  \addplot[
    color=#2,
    mark=#3,
    mark size=1.7pt,
    line width=0.75pt,
    forget plot,
    mark options={solid, fill=#2, draw=#2},
    error bars/.cd,
    y dir=both,
    y explicit
  ] table[x=x,y=mean,y error=se,col sep=comma] {#1};
}

\providecommand{\edmInfoSeries}[4]{%
  \addplot[color=#2, mark=#3, mark size=1.7pt, line width=0.8pt,
    mark options={solid, fill=#2, draw=#2}]
    table[x=x,y=observed,col sep=comma] {#1};
  \addlegendentry{#4}
}

\providecommand{\edmInfoPoints}[4]{%
  \addplot[color=#2, mark=#3, mark size=1.7pt, only marks,
    mark options={solid, fill=#2, draw=#2}]
    table[x=x,y=observed,col sep=comma] {#1};
  \addlegendentry{#4}
}

\providecommand{\edmLawFit}[2]{%
  \addplot[color=#2, line width=0.9pt, forget plot, no marks]
    table[x=x,y=fit,col sep=comma] {#1};
}
\providecommand{\edmRawPoints}[4]{%
  \addplot[color=#2, mark=#3, mark size=1.7pt, only marks,
    mark options={solid, fill=#2, draw=#2}]
    table[x=n,y=observed,col sep=comma] {#1};
  \addlegendentry{#4}
}
\providecommand{\edmRawFit}[2]{%
  \addplot[color=#2, line width=0.9pt, forget plot, no marks]
    table[x=n,y=fit,col sep=comma] {#1};
}
\providecommand{\edmExcessPoints}[3]{%
  \addplot[color=#2, mark=#3, mark size=1.7pt, only marks, forget plot,
    mark options={solid, fill=#2, draw=#2}]
    table[x=x,y=excess,col sep=comma] {#1};
}
\providecommand{\edmExcessFit}[3]{%
  \addplot[color=#2, line width=0.9pt, forget plot, no marks, #3]
    table[x=x,y=excess,col sep=comma] {#1};
}

\providecommand{\edmInsetMem}[2]{%
  \addplot[color=#2, line width=0.8pt, no marks]
    table[x=x,y=memorization,col sep=comma] {#1};
}

% Sigmoid band then ramp band: {ylo}{yhi}{xlo}{xmid}{xhi}.
\providecommand{\edmBandsAt}[5]{%
  \path[fill=black!9] (axis cs:#3,#1) rectangle (axis cs:#4,#2);
  \path[fill=black!4] (axis cs:#4,#1) rectangle (axis cs:#5,#2);
}
\providecommand{\edmDashedSeries}[4]{%
  \addplot[color=#2, mark=#3, mark size=1.7pt, line width=0.75pt, dashed,
    mark options={solid, fill=white, draw=#2},
    error bars/.cd, y dir=both, y explicit]
    table[x=x,y=mean,y error=se,col sep=comma] {#1};
  \addlegendentry{#4}
}
\providecommand{\edmDashedSeriesNoLegend}[3]{%
  \addplot[color=#2, mark=#3, mark size=1.7pt, line width=0.75pt, dashed,
    forget plot, mark options={solid, fill=white, draw=#2},
    error bars/.cd, y dir=both, y explicit]
    table[x=x,y=mean,y error=se,col sep=comma] {#1};
}

\providecommand{\edmRatio}[2]{%
  \addplot[color=#2, line width=0.7pt, opacity=0.72, no marks, forget plot]
    table[x=x,y=ratio,col sep=comma] {#1};
}

\providecommand{\edmZoomPoints}[3]{%
  \addplot[color=#2, mark=#3, mark size=1.3pt, only marks, forget plot,
    mark options={solid, fill=#2, draw=#2}]
    table[x=n,y=observed,col sep=comma] {#1};
}


==> figures/pgfplots/imagenet256_styles.tex <==
\providecolor{imagenetDepthTwo}{RGB}{68,1,84}
\providecolor{imagenetDepthFour}{RGB}{59,82,139}
\providecolor{imagenetDepthEight}{RGB}{33,145,140}
\providecolor{imagenetDepthTwelve}{RGB}{94,201,98}
\providecolor{imagenetDepthSixteen}{RGB}{230,205,28}

\providecommand{\imagenetMetricSeries}[4]{%
  \addplot+[
    color=#2,
    mark=#3,
    mark size=1.7pt,
    line width=0.75pt,
    error bars/.cd,
    y dir=both,
    y explicit
  ] table[x=x,y=mean,y error=se,col sep=comma] {#1};
  \addlegendentry{#4}
}

\providecommand{\imagenetMetricSeriesNoLegend}[3]{%
  \addplot+[
    color=#2,
    mark=#3,
    mark size=1.7pt,
    line width=0.75pt,
    forget plot,
    error bars/.cd,
    y dir=both,
    y explicit
  ] table[x=x,y=mean,y error=se,col sep=comma] {#1};
}


==> figures/pgfplots/phase_transition_styles.tex <==
\providecolor{phaseSmall}{RGB}{31,119,180}
\providecolor{phaseMedium}{RGB}{214,39,40}
\providecolor{phaseLarge}{RGB}{44,160,44}
\providecommand{\phasePanelWidth}{0.420\linewidth}
\providecommand{\phaseTwoPanelHeight}{0.34\linewidth}
\providecommand{\phaseCombinedPanelHeight}{0.33\linewidth}
\providecommand{\phaseHorizontalSep}{2.05cm}
\providecommand{\phaseCriticalLine}[2]{%
  \addplot[black!55, densely dashed, forget plot] coordinates {(1,#1) (1,#2)};
}
\providecommand{\phaseInfoSeries}[4]{%
  \addplot+[
    mark=#3,
    mark size=1.45pt,
    line width=0.65pt,
    color=#2
  ] table[x=x,y=observed,col sep=comma] {#1};
  \addlegendentry{#4}
  \addplot+[
    no marks,
    densely dashed,
    line width=0.75pt,
    color=#2,
    forget plot
  ] table[x=x,y=predicted,col sep=comma] {#1};
}
\providecommand{\phaseMemSeries}[3]{%
  \addplot+[
    mark=#3,
    mark size=1.45pt,
    line width=0.65pt,
    color=#2,
    error bars/.cd,
    y dir=both,
    y explicit
  ] table[x=x,y=memorization,y error=se,col sep=comma] {#1};
}

